On Variational Methods for Motion Compensated Inpainting

We develop in this paper a generic Bayesian framework for the joint estimation of motion and recovery of missing data in a damaged video sequence. Using standard maximum a posteriori to variational formulation rationale, we derive generic minimum energy formulations for the estimation of a reconstructed sequence as well as motion recovery. We instantiate these energy formulations and from their Euler-Lagrange Equations, we propose a full multiresolution algorithms in order to compute good local minimizers for our energies and discuss their numerical implementations, focusing on the missing data recovery part, i.e. inpainting. Experimental results for synthetic as well as real sequences are presented. Image sequences and extra material is available at http://image.diku.dk/francois/seqinp.php.

==> numerics.tex <==
\section{Discretization}
\label{sec:mymc-discrete}


\subsection{Some discrete and semi-discrete adjunction relations}
\label{sec:num}

Finite difference schemes are obtained via discretrization or partial
discretisation of the different energies and derivation of gradients
by the use of adjunction mechnisms similar to the ones used in the
previous section.  Wecompute only gradients with respect to the image
variables in this work. 

%
%For the spatial terms, a full discretization can be
%obtainede immediatly, while time discrete discretisations are first
%devised for the terms

Analogous of Prop. \ref{prop:gradadj} holds for finite differences: we
denote respectively $D_{hx_i}^+$, $D_{hx_i}^-$ and $D_{hx_i}^c$ the forward,
backward and central differences operators in direction $x_i$ with step
$h$. Then modulo proper treatement of boundary conditions, the folllowing
adjunction relations hold (via simple transposition):
$$
\left(D_{hx_i}^+\right)^* = -D_{hx_i}^-,\quad
\left(D_{hx_i}^-\right)^* = -D_{hx_i}^+,\quad
\left(D_{hx_i}^c\right)^* = -D_{hx_i}^c
$$


For the time-discrete case, that will be useful in the numerics, we state a
somewhat technical result, that aims at being a semi-discrete analogous to
Prop. \ref{prop:lieadj} under some simplified assumptions, for more general
ones would result in series of complex terms related to boundary conditions
which appear very difficult to manage.
\begin{prop}
  \label{prop:liadjdisc1}
  Let $\varphi$, $\psi : \RR^2\times\RR$ be continuous functions with
  compact support, $h>0$ a real and $(v^h_i)_{i\in\ZZ}$ a family of
  vector fields defined on $\RR^2$ such that the maps $H_i^h = id + h
  v^h_i$ are diffeomorphisms. Let $K_{i+1}^h =
  \left(H_i^h\right)^{-1}$ and $w^h_j = (id - K_j^h)/h$.  Let
  $|JK_j^h|$ be the Jacobian determinant of $K_j^h$, $|JK_j^h| = 1 -
  h\nabla\cdot w^h_j + h^2|Jw^h_j|$ and $\bx=(x,y)$ the spatial
  coordinates. Dropping, for legibility the superscripts $h$, one has
  \begin{multline}
    \sum_{i\in\ZZ}\int_{\RR^2}\left[(\LieDFh{v_i}{\varphi})(\bx,ih)\right] 
    \psi(\bx,ih)\,d\bx
    =
    -\sum_{i\in\ZZ}\int_{\RR^2}\varphi(\bx,ih)\times\\
    \left[\left(\LieDBh{w_{i}}{\psi}\right)(\bx,ih) + \psi(\bx-hw_i(\bx),(i-1)h)
      (\nabla\cdot w_{i} - h|Jw_{i}|)\right]\,d\bx
\end{multline}
\end{prop}
The proof itself follows directy by an elementary application of the
change of variables theorem and proper renaming of
summation/integration variables. More important is to understand the
relations between $(v_i)_i$ and $(w_j)_j$. The motion fields $(hv_i)$
describe the sequence forward motion in ``temporal steps of duration
$h$''. The $v_i$'s are instrinsically dependent on this step, and this
is the reason we started by denoting them $v_i^h$. Now when $(hv_i)_i$
describe the motion in a given sequence $u$, between time $ih$ and
time $(i+1)h$, $(hw_j)_j$ will describe the motion for the sequence
``reversed in time'', between time $(i+1)h$ and time $h$. One has
$(Id+hv_i)^{-1} := Id-hw_{i+1}$ but also $(Id + hv_i)^{-1} = Id - hv_i
+ o(h)$, i.e. $hw_{i+1} = -hv_i + o(h)$. Using this relation and the
direct dependency of $v_i$ and thus $w_j$ in $h$, it is not difficult
to show that when $h\to 0$, we recover, modulo boundary conditions,
the result of Prop. \ref{prop:gradadj}.  Of course, some apparently
severe regularity assumptions were made on the motion from one frame
to the next, ...

What this proposition provides is a coherent temporal discretisation for the
energy gradients $\nabla_uE_3^i$ that were computed in the previous section
by mean of, among others, Prop. \ref{prop:lieadj}. 

\begin{prop}
  \label{prop:liadjdisc}
  Let $\varphi_i, \psi_i:\RR^2\to\RR^k$, $i\in\ZZ$ two families of
  compactly supported functions, $(H_i)_{i\in\ZZ}$ a family of
  diffeomorphims of $\RR^2$ and $(K_j)_{j\in\ZZ}$ the family of
  diffeomorphisms defined by $K_{j+1} = H_i^{-1}$. Denote by $|JK_i$
  the Jacobian determinant of $K_j$. Then
  $$
  \sum_{i\in\ZZ}\int_{\RR^2}\left(\varphi_{i+1}(H_i(\bx))
    -\varphi_i(\bx)\right)\psi_i(\bx)\,d\bx =
  -\sum_{i\in\ZZ}\int_{\RR^2}\phi_i(\bx)
  \left(\psi_i(\bx)-\psi_{i-1}(K_i(\bx))|JK_i(\bx)|\right)\,d\bx.
  $$
\end{prop}
This proposition follows from a straightforward application of the
Change of Variables Theorem as well as a proper renamining of
summation indices. We use it as follow:
given a $\Cc^1$-vector field $v:\RR^2\times\RR\to\RR^2$ with the
associated dynamic
$$
\dot{\x} = v(\bx(t),t),
$$
a ``particle'' at position $\bx$ at time $t_0$ will move at time 
$t_0 + h$ to the position
$$
c(\bx,t_0+h;t_0) := \bx(t_0+t) = \bx + \int_{t_0}^tv(\bx(t),t)\,dt.
$$
Assume that for $h$ small enough, $c(-,t_0+h;t_0)$ is a diffeomorphism
of $\RR^2$.


%  that and functions $\phi$, $\psi:
%c\RR^2\times\RR\to\RR^k$.

In this section we describe in details the numerics used for the pure
inpainting and inpainting/denoising PDEs. The most important terms,
gray-values diffusion and ``gradient''-diffusion, are common to the
two equations, the differences being the bias term $\chi(I-I_0)$ in
the inpainting/denoising equation, and of course its complex boundary
conditions. There is also an important difference in terms of running
time, the pure inpainting algorithm being run only at pixels in the
missing data locus, while the inpainting/denoising algorithm is run on
the entire image sequence!




We will also point out the minor modifications needed for the
discretization of the vector valued image sequences algorithms.

\subsection{Optical Flow}
\label{subsec:of}
At each resolution level, the optical flow algorithm has been
implemented exactly as described in \cite{brox-bruhn-etal:04}. We will
see in subsection~\ref{subsec:flowdiff} that we also compute optical
flow for the reversed-in-time sequence. For that we construct the new
sequence $I_r(x,y,t) = I(x,y,T-t)$ and apply of course the algorithm
mentioned above.

We need to modify the data term of the optical flow algorithm when
dealing with vector valued images, but, as we saw in
section~\ref{subseq:mymc-color}, it boils down to simply add up the
different channel contributions in the resulting equations to solve,
as it is clear from equation~(\ref{eq:broxflowvec}) (by ``data term'',
we mean the first right hand side term of equation
(\ref{eq:broxflowvec})).

\subsection{Spatial Diffusion}
\label{subsec:spatdiff}
We need to discretize the divergence term $\Div(A\nabla I)$. Given a
pixel $s=(i,j,k)$, let us denote $\nu_s$ its spatial 4-neighborhood
$\nu_s = \{(i-1,j,k),(i,j+1,k),(i+1,j,k),(i,j-1,k)\}$. Then
$$
\Div(A\nabla I)_s \approx \sum_{r\in\nu_s}A_{\frac{r+s}{2}}(u(r)-u(s))
$$
where $(r+s)/2$ denotes the midpoint between $r$ and $s$. To compute
$A_{\frac{r+s}{2}}$, we use standard discretizations, as proposed by
Chan and Shen in \cite{chan-shen:01} consider for instance $r =
(i+1,j,k)$, then we estimate $|\nabla I|^2$ at $(r+s)/2$ by
\begin{eqnarray}
  \label{eq:tvs}
  |\nabla I|_{\frac{r+s}2}^2 \!\!&\approx& \!\! (I_{i+1jk}-I_{ijk})^2 +\nonumber\\ 
  \!\!&& \!\!\frac1{16}(I_{i\!+\!1j\!+\!1k}\!-\!I_{i\!+\!1j\!-\!1k}\!+\!I_{ij\!+\!1k}\!-\!I_{ij\!-\!1k})^2.
\end{eqnarray}
% Alternatively, instead of approximating $I_y$ at $(i+1/2,j,k)$ by
% the average of the central differences in $j$ at $(i+1,j,k)$ and
% $(i,j,k)$, we can use a \emph{minmod} of this central differences,
%% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
%% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!  Joachim says there
%% is a serious consistency problem here, I have to check
%% that!!!!!!!!!  !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
%% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
%$$
%I_{y_{i+\frac12jk}}\approx
% \text{minmod}\left(\frac{I_{i+1j+1k}-I_{i+1j-1k}}{2},\frac{I_{ij+1k}-I_{ij-1k}}{2}\right)
%$$
%where the minmod function is defined as
%$$
%\text{minmod}(x,y) = 
%\begin{cases}
%  0&\quad\text{if } xy \leq 0\\
%  x&\quad\text{if } xy >0, |x| < |y|\\
%  y&\quad\text{otherwise.}
%\end{cases}
%$$
%In practice we did not observed significative differences between the
% two schemes. Note also that the first discretization is more
% coherent when dealing with vector valued image sequences, for
% identical finite difference approximations are performed on each
% channel, whereas minmod may choose different approximations for the
% different channels.

\subsection{Motion Adaptive Inpainting}


Recall that at coarsest resolution level, the inpainting is obtained
as solution of equation~(\ref{eq:madapt_motion-grads}) or
equation~(\ref{eq:madapt_motion}). These two equations have identical
spatial terms.  The first equation is solved by gradient descent, the
temporal discretization being the straightforward adaptation of the
one described the next paragraph (we just set the input optical flow
fields to 0). If we choose instead
$$
-\Div\left(\varphi'(|\nabla I|^2)\right) -
\lambda\partial_t\left(\varphi'(I_t^2)I_t\right) = 0,\quad
I_{|_{D^N\backslash\Omega^N}} = I^N_0
$$
then the temporal derivative is discretized in a very similar, but
simpler way, to the spatial divergence since only the two temporal
neighbors are used. Because of the simplicity of this elliptic PDE, it
is solved directly, not using gradient descent, through a fixed-point
strategy in order to cope with the non linearity. Although the first
one seems more natural from the formulation we studied here, there are
no real significative differences at the final result level, which led
us to use the simple one.

\subsection{Flow Line Terms}
\label{subsec:flowdiff}
Of course, the most important terms for our equations are the ones
involving the motion field.  They are rather complex, we will explain
step by step the chosen discretizations.
\begin{myenum}
\item The first term to discretize is
  $$
  \Div\left(B\ddV{I}\vec{V}\right) = \ddV{}\left(B\ddV{I}\right) +
  B\ddV{I}\Div(\vec{v}).
  $$
  The left hand-side of this equation is not easily handled in the
  discretization due to the apparition of cross-derivatives. We have
  therefore chosen to discretize the right-hand side.  We describe
  first the discretization of terms like
  $\ddV{}\left(B\ddV{f}\right)$.  Given a spatio-temporal location
  $\bp=(x,y,t)$, let us denote $\bp^+$ the point following $\bp$ along
  the flow line at $\bp$, i.e. $\bp^+ = \bp + \vec{V}(\bp)$. Let us
  also denote by $\bp^-$ the point \emph{preceding} $\bp$ along the
  flow line at $\bp$, i.e. $\bp = \bp^- + \vec{V}(\bp^-)$, and notice
  that we have $(\bp^+)^- = (\bp^-)^+ = \bp$. Then we introduce two
  finite difference operators, consistent with the approximation we
  made in section \ref{sec:mymc-motiv}, where $f(\bp + \VV)-f(\bp)$
  was replaced by $\ddV{f}$.
  $$
  D^+_{\vec{V}}f(\bp) = f(\bp^+) - f(\bp),\quad D^-_{\vec{V}}f(\bp) = f(\bp)
  - f(\bp^-)
  $$
  (when $\bp^\pm$ is not on the natural image grid, the quantity
  $f(\bp^\pm)$ is of course computed by spatial interpolation,
  bilinear, bicubic, etc...).  Recall that $B$ was defined as
  \begin{eqnarray*}
    B &=& \varphi'\left(\left(\ddV{I}\right)^2 +
      \gamma\left|\ddV{\nabla I}\right|^2\right) \\
    &\approx&
    \varphi'\left(\left(I(\bp^+)-I(\bp)\right)^2 + \gamma\left|\nabla I(\bp^+)
        -\nabla I(\bp)\right|^2\right)\\
    &:=& B(\bp,\bp^+)
  \end{eqnarray*}
  Then the proposed discretization of $\ddV{}\left(B\ddV{f}\right)$ is
  %{\small
  \begin{eqnarray}
    \label{eq:std_flowline_discret}
    D^-_{\vec{V}}(B(\bp,\bp^+)D^+_{\vec{V}}f(\bp)) =
    D^+_{\vec{V}}(B(\bp^-,\bp)D^-_{\vec{V}}f(\bp)) &=&\nonumber\\ 
    B(\bp,\bp^+)(f(\bp^+) - f(\bp))
    + B(\bp^-,\bp))(f(\bp^-)-f(\bp))&&% + B(\bp^-,\bp)f(\bp^-)
  \end{eqnarray}
  %}
\item The location $\bp^+$ is directly available from the flow
  algorithm, but the location $\bp^-$ is not, see figure~\ref{fig:flowline}.
  \begin{figure}[h]
    \centering \includegraphics[width=\two]{images/flowline.eps}
    \caption{A flow line fragment: ambiguity in flow from previous to
      current frame. \label{fig:flowline}}
  \end{figure}
  This information is difficult to obtain, if possible at all (at
  occlusion/disocclusion, and/or other types of singularities for the
  flow field). In order to overcome this problem, we compute also the
  \emph{backward in time} optical flow $\vec{v}_-$ from $I(-,t)$ to
  $I(-,t-1)$ and we estimate $\bp_-$ as $\bp+\vec{v}_-(\bp)$.  From
  now we adopt the notation $\vec{v}_+$ for the forward-in-time flow
  and $\vec{v}_-$ for the backward-in-time flow.  The corresponding
  $B$ functions will be denoted $B_+$ and $B_-$ respectively. We
  obtain
  \begin{multline}
    \label{eq:flowline_fb}
    \ddV{}\left(B\ddV{f}\right)(\bp)\approx B_+(\bp)f(\bp^+)\\
    - (B_+(\bp)+ B_-(\bp))f(\bp) +  B_-(\bp)f(\bp^-).
  \end{multline}
  In the case of vector valued sequences, the same discretization is
  used, replacing $B_\pm$ by its counterpart, as defined in
  section~\ref{subseq:mymc-color}.
  
\item The term $B\ddV{I}\Div(\vec{v})$ must be handled carefully. A
  naive discretization of the form
  $$
  \frac12 B^+(I(\bp^+)-I(\bp))\Div(\vec{v}_+) - \frac12
  B^-(I(\bp)-I(\bp^-))\Div(\vec{v}_-)
  $$
  where $\Div(\vec{v}_\pm)$ is discretized by standard central
  differences, turned out to be unstable (the ``-'' sign in the second
  term of the above formula comes from the fact that $\vec{v}_-$ is
  \emph{backward in time}). This is not totally unexpected since it is
  a sort of ``transport'' term. We favor the ``best available''
  information, i.e. the one for which the difference between the
  information at $\bp$ and its two flow lines neighbors is minimal. We
  use either $\bp^+$ or $\bp^-$ according to the value of $B_\pm$:
  \begin{equation}
    \label{eq:Bchooser}
    B\ddV{I}\Div(\vec{v})(\bp)\approx
    \begin{cases}
      B^+D^+_{\vec{V}}I(\bp)\Div(\vec{v}_+),&\text{if }B_+ > B_-\\
      -B^-D^-_{\vec{V}}I(\bp)\Div(\vec{v}_-),&\text{otherwise. }
    \end{cases}
  \end{equation}
  since $B_\pm$ provides an explicit measure of the match between the
  information at location $\bp$ and $\bp^\pm$, not only gray level
  variation, but also gradient variation, a low value of $B_\pm$
  corresponding to a poor match, while a large value correspond to a
  good one.
  
\item We explain now the discretization of the higher order terms.
  The first one we treat is
  $$
  \Div\left(\ddV{}\left(B\ddV{\nabla I}\right)\right).
  $$
  Write it as $\partial_x K_1 + \partial_y K_2$ where
  $$
  K_1 = \ddV{}\left(B\ddV{I_x}\right),\quad K_2 = \ddV{}\left(B\ddV{I_y}\right)
  $$
  For each of the spatial derivatives $\partial_x K_1$ and $\partial_y
  K_2$, we use standard central differences, at grid points,instead of
  central differences at half-grid points. The latter involves a large
  amount of interpolations, for both image and flow values, and we
  observed experimentally a loss of accuracy.  We detail here the
  computations for $\partial_x K_1(\bp)$ For a given spatio-temporal
  location $\bp$, let $\bp_E = \bp + (1,0,0)$, the ``east'' neighbor
  of $\bp$, $\bp_W = \bp + (-1,0,0)$, its ``west'' neighbor. Then
  $\partial_x K_1(\bp) \approx \frac{1}{2}(K_1(\bp_E) - K_1(\bp_W))$.
  Using the discretization given in~(\ref{eq:flowline_fb}), we have
  \begin{eqnarray*}
    K_1(\bp_E)&\approx& B_+(\bp_E)I_x(\bp_E^+) - (B_+(\bp_E)+B_-(\bp_E))I_x(\bp_E)+ \\
    &&B_-(\bp_E)I_x(\bp_E^-).
  \end{eqnarray*}
  The derivative $I_x$ is also approximated by standard central
  differences. Similar discretizations are used for $K_1(\bp_W)$, the
  term $\partial_y K_2$ being also approximated as
  $\frac12\left(K_2(\bp_N)-K_2(\bp_S)\right)$, where $\bp_N$ and
  $\bp_N$ denote the ``north'' and ``south'' neighbor points of $\bp$
  on the grid.
  
\item Similar approximations are used for the remaining term
  $$
  \Div\left(B\ddV{\nabla I}\Div(\vec{v})\right) =
  \partial_x\!\!\left(B\ddV{I_x}\Div(\vec{v})\right) +
  \partial_y\!\!\left(B\ddV{I_y}\Div(\vec{v})\right)
  $$
  i.e. standard central differences in $x$ and $y$ for evaluating the
  divergence, using this time~(\ref{eq:Bchooser}) for the terms
  $B\ddV{I_z}\Div(\vec{v})$, $z=x,y$. We have concentrated on the
  latter form, i.e.  selecting forward or backward flow line
  differences for the $\ddV{I_z}$ terms (and the selection of either
  forward or backward flow) according to the values of the function
  $B$.
\end{myenum}




\subsection{Inpainting-Denoising}
\label{sec:id}
As we mentioned in the introduction of that section, added to the
diffusion terms, there is also a bias term in the inpainting-denoising
equation, namely $\chi(I-I_0)$.  Its discretization is trivial. Much
more complicated are the natural boundary conditions, as we saw in
equation~\ref{eq:natbc}. Depending on image and flow conditions, they
may even do not have any sense! Therefore more ad hoc, but also more
realistic conditions were needed.  It has consisted in not using
motion when we would leave the sequence domain. In such situation,
only spatial regularization is applied. Boundary conditions for
spatial regularization are just the usual reflecting boundary
conditions.

However, in the actual state of the algorithm, the computational time
for the inpainting/denoising purpose is \emph{prohibitive}. When a
couple of minutes are sufficient to treat the \texttt{Yosemite}
sequence (see the Experiment section) it can take several hours for
the inpainting denoising. This has led us not to present examples of
denoising/inpainting.

\subsection{Missing Data Locus and Multiresolution}
\label{sec:mask}

So far, we have not mentioned the treatment of the missing data locus
with respect to our multiresolution algorithm. At a pyramid level $p >
0$ the \emph{known} image data comes from the data at level 0 after
filtering and downsampling/interpolation (the latter is needed if we
choose arbitrary scaling factors between pyramid levels, what we
indeed do).  The problem with the missing data locus, as we use it, is
that this is a binary image, i.e. a subset of the domain, and should
remain so after downsampling at a given resolution level. We present
here a simple way of downsampling this set.

Call $D_p$ the discrete image domain at resolution level $p \geq 0$
and $\pi_p$ the downsampling operator:
$$
\pi_p(D_0) = D_p,\quad \pi_p(I:D_0\to \RR) = I_p:D_p\to \RR.
$$
A way to be on the ``safe side'' would be to define the missing data
locus $\Omega_p$ at resolution $p$ by
$$
\Omega_p = \{(x,y,t)\in D_p|\pi_p^{-1}(x,y,t)\cap\Omega \not= \emptyset\}
$$
i.e. any pixel value which incorporates some of the known corrupted
(missing) data should be marked as bad and its location therefore
added to the missing data locus at that resolution.  In practice this
is implemented the following way. Using the characteristic function
$\chi$ of $D\backslash\Omega$, we downsample it to a function $\chi_p$
using our downsampling operator $\pi_p$ and we define $\Omega_p$ by
$$
\Omega_p = \{(x,y,t)\in D_p|\chi_p(x,y,t) < 1\}.
$$
The filters used for the downsampling operation were small smoothing
kernels, more precisely truncated Gaussians, whose diameter support is
of the order of $p\times$scaling-factor, so that $\Omega_p$ does not
becomes ``too big''.


